Train Once for All: A Transitional Approach for Efficient Aspect Sentiment Triplet Extraction

Aspect-Opinion Pair Extraction (AOPE) and Aspect Sentiment Triplet Extraction (ASTE) have drawn growing attention in NLP. However, most existing approaches extract aspects and opinions independently, optionally adding pairwise relations, often leading to error propagation and high time complexity. To address these challenges and being inspired by transition-based dependency parsing, we propose the first transition-based model for AOPE and ASTE that performs aspect and opinion extraction jointly, which also better captures position-aware aspect-opinion relations and mitigates entity-level bias. By integrating contrastive-augmented optimization, our model delivers more accurate action predictions and jointly optimizes separate subtasks in linear time. Extensive experiments on 4 commonly used ASTE/AOPE datasets show that, while performing worse when trained on a single dataset than some previous models, our model achieves the best performance on both ASTE and AOPE if trained on combined datasets, outperforming the strongest previous models in F1-measures (often by a large margin). We hypothesize that this is due to our model's ability to learn transition actions from multiple datasets and domains. Our code is available at https://anonymous.4open.science/r/trans_aste-8FCF.

==> old-intro.tex <==
\section{Introduction}
Sentiment analysis, the computational study of opinions, emotions, and attitudes in text, has emerged as a vital research area with applications spanning from business to social sciences \cite{Pang2002, Liu2012, Cambria2016, wang2025dlf}. Aspect-Based Sentiment Analysis (ABSA) is a fine-grained sentiment analysis task that identifies specific aspects in text and analyzes the sentiments linked to them \cite{Hu2004}. It involves subtasks such as: \textbf{\textit{Aspect Extraction (AE)}}: Identifying mentioned aspects. \textbf{\textit{Opinion Extraction (OE)}}: Extracting opinion terms related to aspects. \textbf{\textit{Aspect-Opinion Pair Extraction (AOPE)}}: Extracting aspect-opinion pairs. \textbf{\textit{Aspect-Sentiment Triplet Extraction (ASTE)}}: Identifying aspect, opinion, and sentiment polarity triplets.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=\linewidth]{display.png}
\caption{For the sentence 'Gourmet food is delicious. Good service, but not so welcoming,' this example demonstrates the processing steps in both classic and transitional methods for extracting aspect-opinion pairs and tagging sentiment polarity. AE stands for Aspect Extraction, OE for Opinion Extraction, \textcolor{customgreen}{POS} represents positive sentiment, and \textcolor{rr}{NEG} represents negative sentiment.
}
\label{d}
\end{center}
\end{figure}
Classic ABSA approaches often use a pipeline architecture, performing subtasks like aspect extraction (AE) and opinion extraction (OE) separately. For instance, in the sentence: “\textit{Gourmet food is delicious. Good service, but not so welcoming.},” AE identifies \textbf{\textcolor{blueish}{gourmet food}} and \textbf{\textcolor{blueish}{service}} as aspects, while OE extracts \textbf{\textcolor{orange}{delicious}}, \textbf{\textcolor{orange}{good}}, and \textbf{\textcolor{orange}{not so welcoming}} as opinions. These outputs are combined to form aspect-opinion pairs, with sentiment tagging assigning polarities to create triplets. Past studies have generally achieved satisfactory performance 
% \fly{No need to write this score} 
on aspect and opinion extraction \cite{jiang2023semanticallyenhanceddualencoder, 10.1007/978-3-031-25198-6_8, chakraborty2024aspectopiniontermextraction}. 

Adding the according sentiment tags with pair, ASTE is the most integrated task for aspect-based sentiment analysis that has seen the development of diverse models leveraging various methodologies. 
% \fly{there is no parallelism with the previous content and \' Furthermore\'.} 
Pipeline-based approaches, such as Peng-Two-stage \cite{Peng_Xu_Bing_Huang_Lu_Si_2020}, decompose the task into multiple stages for modular refinement. Sequence-to-sequence frameworks like BARTABSA \cite{yan-etal-2021-unified} employ pretrained transformers to generate triplets flexibly. Sequence-tagging methods, including GTS \cite{wu2020grid} and JET-BERT \cite{xu2020position}, annotate tokens for precise identification of relationships. Machine Reading Comprehension (MRC)-based models, such as COM-MRC \cite{zhai2022mrc} and Triple-MRC \cite{zou2024multi}, reframe the task as query answering for efficient extraction. Graph-based approaches such as EMC-GCN \cite{chen2022enhanced}, BDTF \cite{chen2022enhanced}, and DGCNAP \cite{li2023dual} use graph structures to capture semantic and syntactic interactions. Tagging schema-based models, exemplified by STAGE-3D \cite{liang2023stage}, use hierarchical schemas for multi-level extraction, while lightweight models like MiniConGTS \cite{sun-etal-2024-minicongts} focus on efficiency with reduced computational costs.

Although previous studies have shown satisfactory results for individual entity extraction, performance on pair and triplet extraction remains suboptimal, with state-of-the-art (SOTA) scores in the 60s and 70s \cite{sun-etal-2024-minicongts}. Two key challenges contribute to this gap: 
(1) Disconnected Aspect-Opinion Extraction: Opinions are often extracted independently from their corresponding aspects in previous studies \cite{liang2023stage, sun-etal-2024-minicongts}. While relationships can be added as an auxiliary factor to assist pair extraction \cite{liu2022mrce, 10.1007/978-3-031-25198-6_8}, this approach loses critical contextual information by treating aspects and opinions as separate entities. This limits the effectiveness of many token-based extraction methods. 
(2) Time Complexity with Longer Sequences: Methods using 2D matrix tagging \cite{liang2023stage, sun-etal-2024-minicongts} to capture relationships between tokens face significant increases in time complexity as the length of the token sequence increases. This computational burden restricts their scalability, especially for longer texts in practical applications. As an overview, the critical contributions of our study are as follows:
\begin{itemize}
\item We propose transition pipelines \textbf{Trans-AOPE} and \textbf{Trans-ASTE} that achieve linear time complexity $O(n)$, marking them as the first to extract aspect-opinion pairs based on relational aspects rather than using relational factors as supplementary references or confirmation.
\item Building on the proposed transitional framework, we introduce a contrastive-augmented optimization method to enhance model efficiency. We conduct experiments to investigate how contrastive learning influences the optimization process, offering detailed insights into its impact on convergence and performance.
\item We introduce \textit{OmniTrain} to train the baseline models, Trans-AOPE, and Trans-ASTE over multiple datasets simultaneously so that the models can achieve optimal performance without individual dataset training. By learning patterns across datasets, this approach helps capture the essential features of aspect-opinion pairs and aspect-sentiment triplets for better generalization.
\end{itemize}



